Holographic approach to transport in dense QCD matter

The transport properties of dense QCD matter play a crucial role in the physics of neutron stars and their mergers, but are notoriously difficult to study with traditional quantum field theory tools. Specializing to the case of unpaired quark matter in beta equilibrium, we approach the problem through the machinery of holography, in particular the V-QCD and D3-D7 models, and derive results for the electrical and thermal conductivities and the shear and bulk viscosities. In addition we compare the bulk to shear viscosity ratio to the speed of sound and find that it violates the so-called Buchel bound. Our results differ dramatically from earlier predictions of perturbative QCD, the root causes and implications of which we analyze in detail.

==> hydroconds.tex <==

%Some of the transport properties that we will obtain in the holographic calculation can already be derived by solving relativistic hydrodynamic equations, as expected from the fluid/gravity correspondence. In addition, this analysis will also help us to interpret our results. 
%In this section, we are going to discuss the relation between different transport coefficients derived from the relativistic hydrodynamic expansion; therefore, there is no holography yet. Some of the relations that we are going to obtain will be recovered in our holographic setup. On the other hand, we will need some others to complete the holographic computation.
%In the presence of a background metric $g_{\mu\nu}$ and gauge field $A_\mu$, the conservation equations for the energy-momentum tensor $T_{\mu\nu}$ and current $J^\mu$ read:
%\begin{equation}
%    \nabla_{\mu}T^{\mu\nu} = F^{\nu\lambda}J_\lambda, 
%    \quad \nabla_\mu J^\mu
%\end{equation}
%In the hydrodynamic description the dynamical variables are reduced to the temperature $T$, chemical potential $\mu$ and velocity $u^\mu$, ($u^\mu u_\mu=-1$) so the number of conservation equations matches with the number of variables. The energy-momentum and the current are local functionals of these variables and their derivatives, as fixed by the constitutive relations, that take the form of an expansion in small derivatives. The general form is
%\be
%\begin{aligned}
% T^{\mu\nu}& =(\varepsilon+p)\  u^\mu u^\nu+p \ g^{\mu\nu}+\tau^{\mu\nu},\\[2mm]
%J^\mu & =\rho\ u^\mu+\nu^\mu \ .
%\end{aligned}
%\ee
%In the previous expression, the non-derivative terms are the contributions from ideal hydrodynamics: $p$ is the pressure, $\varepsilon$ is the energy density and $\rho$ the charge density. On the other hand, $\tau^{\mu\nu}$ and $\nu^{\mu}$ contain derivatives of the fields. We choose to work in the Landau frame:
%\be
% u_{\mu} \tau^{\mu\nu}=0,\quad u_{\mu}\nu^{\mu}= 0.
%\ee
%One should also note that $T^{\mu\nu} = T^{\nu\mu}$.
%If there is neither background magnetic field nor other sources of parity breaking, the most general constitutive relations compatible with the second law of thermodynamics are, to first order in derivatives
%\be\begin{aligned}
% \tau^{\mu\nu}&=-\eta \Sigma^{\mu\nu}-\zeta P ^{\mu\nu} \nabla_\lambda u^\lambda,\\[2mm]
%\nu^\mu &=\sigma \left( E^\mu-T P^{\mu\nu}\nabla_\nu \left( \frac{\mu}{T}\right)\right).
%\end{aligned}
%\ee
%Here we have introduced the projector transverse to the velocity, given by $P^{\mu\nu}=g^{\mu\nu}+u^\mu u^\nu$, the shear tensor
%\be
% \Sigma^{\mu\nu}=P^{\mu\alpha} P^{\nu\beta}\left(\nabla_\alpha u_\beta+\nabla_\beta u_\alpha-\frac{2}{3} g_{\mu\nu}\nabla_\lambda u^\lambda \right),
%\ee
%and the electric field $E^\mu=F^{\mu\nu}u_\nu$. The coefficients $\eta$, $\zeta$ and $\sigma$ are the shear and bulk viscosities and the conductivity, respectively.
%Until this point, we have kept everything quite general. Let us now consider a system in absence of external sources, that is to say $g_{\mu\nu} = \eta_{\mu\nu}$ and $A_\mu = 0$. In such scenario, the equilibrium configuration of the fluid at rest is simply given by:
%\bea
% T&= & T_0,\quad \mu=\mu_0,\quad \varepsilon(T_0,\mu_0)=\varepsilon_0,\quad p(T_0,\mu_0)=p_0 \\
% u^0_0 & = & 1,\qquad u^i_0=0, \qquad i=1,2,3 \ .
%\eea
%Next we perturb the system slightly out of equilibrium and find the response. We are interested in homogeneous transport, so it will be sufficient to consider small time dependent perturbations of the external sources
%\be\begin{aligned}
% g_{\mu\nu} &=\eta_{\mu\nu}+\epsilon \ \delta h_{\mu\nu}(t) + \OO(\epsilon^2),\\[2mm]  A_\mu&=\epsilon \ \delta a_\mu(t)+\OO(\epsilon^2).
%\end{aligned}\ee
%Consequently, a small homogeneous change is introduced in the hydrodynamic variables:
%\be\begin{aligned}
% T &= T_0+\epsilon\ \delta T(t) + \OO(\epsilon^2), \quad \mu=\mu_0+\epsilon \ \delta \mu(t)+ \OO(\epsilon^2), \\[2mm] u^0 &= 1,\quad  u^i=\epsilon\  \delta v^i(t) + \OO(\epsilon^2), \qquad i=1,2,3.
%\end{aligned}\ee
%Plugging these expressions into the hydrodynamic equations and keeping only the terms linear in $\epsilon$, we end up with a set of linear equations for $\delta T(t)$, $\delta\mu(t)$ and $\delta v^i(t)$, sourced by $\delta h_{\mu\nu} (t)$ and $\delta a_\mu (t)$. 
%We can then use an expansion in Fourier modes and solve for a fixed value of the frequency $\omega$. 
%The value of the energy-momentum tensor and the current in the presence of the external sources is obtained by introducing the solutions for the thermodynamic variables back in the constitutive relations and expanding to $O(\epsilon)$. We will only keep non-vanishing vector sources $\delta h_{0i}$ and $\delta a_i$.
%and $O(\omega)$. 
%%*******************************
%\begin{comment}
In order to compute transport coefficients, we turn to Kubo formulas, which define the value of the transport coefficients as the variation of the conserved currents with respect to the external sources, once contact terms have been properly subtracted. Let us focus first in the conductivities, namely:
\begin{itemize}
    \item Electrical conductivity:
\be \label{eq:electricalConductivity}
 \sigma^{ij}=\lim_{\omega\to 0}\frac{1}{i\omega} \left( \frac{\rho_0^2}{\varepsilon_0+p_0} \delta^{ij}+\frac{\delta J^i }{\delta (\delta a_j)}\right)= \sigma \delta^{ij}.
\ee    
\item Momentum - charge conductivity:
\be \label{eq:momentunchargeConductivity1}
 T_0\ \hat{\alpha}^{ij}=\lim_{\omega\to 0}\frac{1}{i\omega} \left( \rho_0\delta^{ij}+\frac{\delta J^i }{\delta (\delta h_{0j})}\right)=0.
\ee
\be \label{eq:momentunchargeConductivity2}
 T_0\ \hat{\alpha}^{ij}=\lim_{\omega\to 0}\frac{1}{i\omega} \left( \rho_0\delta^{ij}+\frac{\delta T^{0i} }{\delta (\delta a_j)}\right)=0.
\ee
\item Momentum - momentum conductivity:
\be \label{eq:momentunmomentumConductivity1}
 T_0\ \hat{\kappa}^{ij}=\lim_{\omega\to 0}\frac{1}{i\omega} \left( \varepsilon_0\delta^{ij}+\frac{\delta T^{0i} }{\delta (\delta h_{tj})}\right)= 0.
\ee
\end{itemize}

Note that from \eqref{eq:electricalConductivity} to \eqref{eq:momentunmomentumConductivity1} we conclude that the electrical conductivity is the only one which is not zero in this setup. In addition to that, the heat current is defined by subtracting the motion of free particles from the energy current. That is to say:
\be \label{eq:heatCurrent}
 Q^i = T^{0i} -\mu\ J^{i} \ .
\ee
From \eqref{eq:heatCurrent} we can extract the thermoelectric and heat transport coefficients as follows:
\begin{itemize}
\item Thermoelectric conductivity
\be
 \alpha^{ij}=\hat{\alpha}^{ij}-\frac{\mu_0}{T_0} \sigma^{ij}=-\frac{\mu_0}{T_0} \sigma \delta^{ij} \ ,
\ee
\item Heat conductivity
\be
 \bar{\kappa}^{ij}=\hat{\kappa}^{ij}-2\mu_0  \alpha^{ij}+\frac{\mu^2_0}{T_0} \sigma^{ij}=\frac{\mu^2_0}{T_0} \sigma \delta^{ij} \ .
\ee
\end{itemize}

We can group all the conductivities together in a single conductivity matrix giving the electric and heat response to an external electric field and a temperature gradient
\be \label{eq:conductivityMatrix_Definition}
 \left(\begin{array}{c} J^i \\ Q^i \end{array}\right)=\left( \begin{array}{cc} \sigma^{ij} & \alpha^{ij} \\ T_0\ \alpha^{ij} & \bar{\kappa}^{ij} \end{array} \right)\left( \begin{array}{c} E_j \\ -\nabla_j T\end{array}\right) \ ,
\ee
which in our case reads
\be \label{eq:conductivityMatrix_ourCase}
 \left( \begin{array}{cc} \sigma^{ij} & \alpha^{ij} \\ T_0\  \alpha^{ij} & \bar{\kappa}^{ij} \end{array} \right)=\sigma \delta^{ij}\left( \begin{array}{cc} 1 & -\frac{\mu_0}{T_0} \\ -\mu_0 & \frac{\mu^2_0}{T_0} \end{array} \right) \ .
\ee

In many physical situations (for instance, if the system is bounded), there is transport of heat without an electric current. This can only happen if there is a balance between electric field and temperature gradient. Imposing the condition $J^i=0$, we get from \eqref{eq:conductivityMatrix_Definition} that
\be
 E_i= \vartheta_i^{\ j} \nabla_j T \ , 
\ee
where $\vartheta=\sigma^{-1}\alpha$ are the Seebeck coefficients. In our case, using \eqref{eq:conductivityMatrix_ourCase} we end up with:
\be
 \vartheta_i^{\ j} =-\frac{\mu}{T} \delta_ i^{\ j} \ .
\ee
Because of that the heat current becomes
\be
 Q^i= -\kappa^{ij}\nabla_j T\ ,
\ee
where the previous expression defines the thermal conductivity, which is given by $\kappa=\bar{\kappa}- T_0 \alpha \sigma^{-1} \alpha$. Note that in this case there is an exact cancellation
\be
 \kappa^{ij}=0 \ .
\ee
%%*******************************
%Having stated the expressions and relations between these conductivities, let us turn now to specify the linear growing of the perturbations with time. Concretely, considering the explicit dependence of the currents on the sources \ack{JGS: indices up and down, is that a problem?}:
\be
\begin{aligned}
J^i &= -\delta^{ij}\left(\frac{\rho_0^2}{\varepsilon_0+p_0 }\ \delta a_j+\rho_0\ \delta h_{0j} + \sigma\  \partial_t\delta a_j\right),\\[2mm]
T^0_{\ i} &= -\rho_0\ \delta a_i - (\varepsilon_0 + p_0)\  \delta h_{0i}.
\end{aligned}
\ee
In the following we will assume that all thermodynamic quantities are given by their equilibrium values and drop the ``$0$'' label. The heat current is defined by subtracting the motion of free particles from the energy current. That is to say:
\be \label{eq:heatCurrent}
Q^i = \delta^{ij}T^0_{\ j} -\mu\ J^{i}.
\ee
In order to extract the DC transport coefficients we will study the response to a constant electric field and temperature gradient. This corresponds to the  following choice for the perturbations:
\be\label{eq.linearintimesources}
\delta a_i = -t(E_i -\mu \zeta_i),\qquad \delta h_{0i} = -t\zeta_i,
\ee
where $\zeta_i = -\nabla_i T/T$. We find the following expressions for the currents
\be\label{eq:currentLinearInTime}
\begin{split}
J^i &= \delta^{ij}\left(\frac{\rho}{\varepsilon+p}\ t\left[(\varepsilon+p-\mu \rho)\zeta_i +\rho E_i\right]\right)\\ &\qquad\qquad\qquad\qquad\qquad\qquad +\sigma\delta^{ij} (E_j-\mu\zeta_j),\\[2mm]
T^0_{\ i}&=t\left[\rho E_i+(\varepsilon+p-\mu\rho)\zeta_i\right].
\end{split}
\ee
We observe terms that grow linearly in time, those correspond to the acceleration of free components of the fluid due to the forces produced by the electric field and temperature gradient. We can prepare the system in such a way that those two forces compensate each other, so the total acceleration vanishes. This can be accomplished imposing the following relation between the sources
\be \label{eq:relationSources}
\rho E_i + T s\ \zeta_i = 0,
\ee
and using the thermodynamic relation $\varepsilon + p - \mu p = T s$. 
%Note that, for later reference, in \eqref{eq:relationSources} we have dropped the subscript $0$ standing for the equilibrium values. 
%Now, if we identify $\zeta_i = -\nabla_i T/T$, the Seebeck coefficient is
%\be
%\vartheta_i^{\ j}=\frac{s_0}{\rho_0}\delta_i^{\ j}\equiv S \delta_i^{\ j},
%\ee
%which is the usual value for the Seebeck coefficient $S$: entropy per unit charge. 
If we impose \eqref{eq:relationSources} in \eqref{eq:currentLinearInTime}, we find that the terms linear in time vanish, and the charge and heat current become
%%*******************************
%\begin{comment}
\be
\begin{split}
&J^i=\delta^{ij}\left( \sigma E_j-\mu_0\sigma \zeta_j\right),\\
&Q^i=T^0_{\ j}-\mu_0 J^i=-\mu_0\sigma  E_i+\mu_0^2\sigma \zeta_i.
\end{split}
\ee
From the last expression it is easy to see that, upon the identification $\zeta_i = -\nabla_iT / T$, one recovers the result obtained before fixing the linear in time growth of the sources \eqref{eq:conductivityMatrix_ourCase}. On the top of that, one can further use \eqref{eq:relationSources} to solve $\zeta_i$ in terms of $E_i$, and get for the currents:
%%*******************************
\be
\begin{array}{lll}
J^i & \displaystyle = \sigma\frac{\varepsilon+p}{Ts}\delta^{ij}E_j&\displaystyle=-\sigma\frac{\varepsilon+p}{\rho} \delta^{ij}\zeta_j,\\[4mm]
Q^i &\displaystyle=-\mu\sigma\frac{\varepsilon+p}{Ts}\delta^{ij} E_j&\displaystyle=\mu\sigma\frac{\varepsilon+p}{\rho}\delta^{ij}\zeta_j.
\end{array}
\ee
Even though the total acceleration vanishes, and the fluid remains at rest (the momentum density is zero $T^0_{\ i}=0$), there is a net transport of charge and heat. The first could be visualized as a separation between positive and negative charges moving in opposite directions. This motion would also take elements of the fluid from regions of higher temperature to regions of lower temperature and vice versa, thus producing the heat current.

In conclusion, the hydrodynamic analysis leads to the following expressions for the DC electric and thermal conductivities in a steady state
%where again we drop the subscript $0$ for later reference:
\be\label{eq:DCelectricandthermaconduc}
 \widetilde{\sigma}^{ij}= \sigma\frac{\varepsilon+p}{Ts}  \delta^{ij} \ , \  \widetilde{\kappa}^{ij}=\frac{\mu}{T}\sigma\frac{\varepsilon+p}{\rho}\delta^{ij} \ .
\ee
Note that both transport coefficients are determined by a single quantity, $\sigma$, corresponding to the conductivity term in the constitutive relations of the current. The dependence on $\sigma$ drops from the ratio, which might be considered as analogous to the Wiedemann-Franz law derived from the Drude model, where it is the dependence on the mean free time that drops.


%\end{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

